Model Predictive Control with Visibility Graphs for Humanoid Path Planning and Tracking Against Adversarial Opponents

In this paper we detail the methods used for obstacle avoidance, path planning, and trajectory tracking that helped us win the adult-sized, autonomous humanoid soccer league in RoboCup 2024. Our team was undefeated for all seated matches and scored 45 goals over 6 games, winning the championship game 6 to 1. During the competition, a major challenge for collision avoidance was the measurement noise coming from bipedal locomotion and a limited field of view (FOV). Furthermore, obstacles would sporadically jump in and out of our planned trajectory. At times our estimator would place our robot inside a hard constraint. Any planner in this competition must also be be computationally efficient enough to re-plan and react in real time. This motivated our approach to trajectory generation and tracking. In many scenarios long-term and short-term planning is needed. To efficiently find a long-term general path that avoids all obstacles we developed DAVG (Dynamic Augmented Visibility Graphs). DAVG focuses on essential path planning by setting certain regions to be active based on obstacles and the desired goal pose. By augmenting the states in the graph, turning angles are considered, which is crucial for a large soccer playing robot as turning may be more costly. A trajectory is formed by linearly interpolating between discrete points generated by DAVG. A modified version of model predictive control (MPC) is used to then track this trajectory called cf-MPC (Collision-Free MPC). This ensures short-term planning. Without having to switch formulations cf-MPC takes into account the robot dynamics and collision free constraints. Without a hard switch the control input can smoothly transition in cases where the noise places our robot inside a constraint boundary. The nonlinear formulation runs at approximately 120 Hz, while the quadratic version achieves around 400 Hz.

==> Sections/S0_nomenclature.tex <==
%%% Section needed to define variables

\nomenclature{$p$}{probability of latching success for a position.}
\nomenclature{$r$}{length from cutout center to nearest hole edge.}
% \nomenclature{$r'$}{length from assembly center to cutout center.}
\nomenclature{$R$}{radial length of cutout.}
\nomenclature{$\rho$}{length from blade assembly center to blade tips.}
\nomenclature{$\tau$, $u$}{torque and control input, respectively.}
% \nomenclature{$\theta$}{angle between $r'$ and nearest edge.}
\nomenclature{$\omega$}{orientation misalignment between latch and pattern.}
\nomenclature{$\vartheta$}{angle between edges defining holes in pattern.}
\nomenclature{$W$}{length from blade assembly center to outer limit.}
\nomenclature{$x$, $y$}{Cartesian coordinates of $r$ and $\theta$.}
\nomenclature{*}{indicates an optimal parameter.}
\nomenclature{$\Psi$}{misalignment tolerance metric.}
\nomenclature{$h$}{height from tips of blades to base.}
\nomenclature{$q$, $\dot{q}$, $\ddot{q}$}{joint angle, velocity, and acceleration, respectively.}
\nomenclature{$K$, $M$}{joint controller gains and mass matrix, respectively.}
\nomenclature{$c$, $g$, $b$}{Coriolis, gravity, and damping terms, respectively.}
\nomenclature{$J$, $F$}{Jacobian and end effector forces, respectively.}

\printnomenclature

==> Sections/S2z_line_interpolation.tex <==
\section{line interpolation}
\label{sec:line_interpolation}
\hl{saw this in the previous section as well so maybe just delete this section?}
The line interpolation generates a well-defined trajectory by assigning a time stamp to the path. There are multiple ways to do the interpolation. The simplest is linear interpolation which is \(C_0\) continuous. We can also use Cubic Hermite Spline to make a \(C_1\) continuous trajectory. Besides, Quintic Bézier Curve can be used for \(C_2\) continuous trajectory. For humanoids, rotating and moving together is not efficient. When it is moving forward reaching out the leg, it is difficult to turn it orientation. Therefore, the linear interpolation suit most for us. Besides, linear interpolation keeps the shortest path which maintains obstacle free property and help robot go to the goal faster.


